Termination of lambda-calculus with the extra Call-By-Value rule known as assoc

In this paper we prove that any lambda-term that is strongly normalising for beta-reduction is also strongly normalising for beta,assoc-reduction. assoc is a call-by-value rule that has been used in works by Moggi, Joachimsky, Espirito Santo and others. The result has often been justified with incomplete or incorrect proofs. Here we give one in full details.

==> LJQ-old.tex <==
\section{\lLJQ}

\begin{definition}[\lLJQ]
$$
\begin{array}{lll}
V, V' & ::=     & x        
        \sep    \l x.M                        
        \sep    \JCrxV{V}{x}{V'}
\\
M,N,P & ::=     & \cst{V}       
                        \sep   \ap{x}{V}{y}{N} 
                        \sep    \JCrx{V}{x}{N}
                        \sep   \letin{M}{x}{N}
\end{array}
$$

The typing rules are shown in Fig.~\ref{Fig:LJQterms}. Derivability,
in the typing system of \lLJQ, of the sequents $\Deriv{\Gamma} V A$
and $\Deri{\Gamma} M A$, is denoted $\DeriLJQv{\Gamma} V A$ and
$\DeriLJQ{\Gamma} M A$, respectively.

\begin{figure}[!h]
{\small
$$
\begin{array}{|cc|}
\hline&\\
\infers{\strut}{\Deriv{\Gamma,x\col A} x A}{}&\quad \infers {\Deriv
  {\Gamma} V A}
{\Deri \Gamma {\cst V} A}{}\\
&\\
\infers{\Deri {\Gamma,x\col A} M B}{\Deriv \Gamma{\l x.M}{A\arr B}}{}
&\quad
\infers{\Deriv {\Gamma,x\col A\arr B} V {A}\quad \Deri {\Gamma,x\col
    A\arr B,y\col B} N C}{\Deri
{\Gamma,x\col A\arr B} {\ap x V y N} C}{}\\
&\\
\infers {\Deriv \Gamma V A\quad
\Deriv {\Gamma,x\col A} {V'} B}{\Deriv \Gamma {\JCrxV{V}{x}{V'}} B}{}
&\quad \infers {\Deriv \Gamma V A\quad
\Deri {\Gamma,x\col A} N B}{\Deri \Gamma {\JCrxV{V}{x}{N}} B}{}\\
&\\
&\quad \infers {\Deri \Gamma M A\quad
\Deri {\Gamma,x\col A} N B}{\Deri \Gamma {\letin M x N} B}{}\\
&\\
\hline
\end{array}
$$}
\caption{Typing system of \lLJQ}
\label{Fig:LJQterms}
\end{figure}

The reduction system, also called $\lLJQm$, is shown in Fig.~\ref{Fig:LJQredbis}.
\begin{figure}[!h]
$$
\begin{array}{|lll|}
\upline
&\flush
\letin{\cst{\l x.M}}y{\ap y V z P}\flush&\Rew{}\letin {\letin {\cst V} x M} z
P\quad\mbox{if
$y\notin \FV V\cup \FV P$}\\
        &\flush       \letin {\cst x} y N\flush&\Rew{}\subst N  y x\\
        &\flush       \letin M y {\cst y}\flush&\Rew{}M
\mmidline
        &\flush\letin {\ap z V y P} x N&\Rew{}\ap z V y {\letin  P x N}\\
        &\flush\letin {\letin {\cst {V'}} y {\ap y V z P}} x N&\Rew{}\letin{\cst {V'}} y {\ap y V z {\letin  P x N}}\\
        &       &\hfill\mbox{if $y\notin \FV V\cup \FV P$}\\
        &\flush\letin {\letin M y P} x N&\Rew{}\letin M y {\letin  P x N}\\
        &       &       \hfill \mbox{if the redex is not one of the
previous rule}\\
        &\flush\letin {\cst {\l y.M}} x N&\Rew{}\JCrx {\lambda y.M} x N
        \mbox{ if $N$ is not an $x$-covalue}
\mmidline
&\JCrxV V x x&\Rew{} V\\
&\JCrxV V x y&\Rew{} y\\
&\JCrxV V x {\l y.M}&\Rew{}{\l y.\JCrx V x M}
\midline
&\JCrx V x {\cst {V'}}&\Rew{}\cst {\JCrxV V x {V'}}\\
&\JCrx V x {\ap x {V'} z P}&\Rew{}\letin {\cst V} x {\ap x {\JCrxV V x {V'}} z {\JCrx
V x P}}\\
&\JCrx V x {\ap {x'} {V'} z P}&\Rew{}{\ap {x'} {\JCrxV {V} x {V'}} z {\JCrx V x P}}\\
&\JCrx V x {\letin M y P}&\Rew{}\letin {\JCrx V x M} y {\JCrx V x P}
\downline
\end{array}
$$
\caption{Reduction rules of \lLJQ}
\label{Fig:LJQredbis}
\end{figure}

\end{definition}

As mentioned earlier, the purpose of this paper is to prove that if $\Deri \Gamma M A$ then $M\in\SN{}$.

\section{Strong normalisation of \lLJQ}
\subsection{An encoding into $\l$-calculus}

\begin{definition}
We extend the notions of value and $x$-covalue into the larger sets of
terms of \emph{pseudo value} $\pv$ and \emph{pseudo $x$-covalue} $\pcv x$,
respectively.  These sets are defined inductively in
Fig.~\ref{fig:pseudocv} and~\ref{fig:pseudov}.  Consequently, a cut
$\letin N x M$ is said to be \emph{pseudo principal} if $N\in\pv$ and $M\in\pcv
x$.
\end{definition}

\begin{figure}[!h]
$$
\begin{array}{|c|}
\upline\\[-6pt]
\infer[x\not\in \FV V\cup\FV M]{\ap x V y M\in\pcv x}{}
\\\\
\infer[x\not\in \FV V]{\JCrx V y M\in\pcv x}{M\in\pcv x}
\qquad
\infer[x\not\in \FV N]{\letin M y N\in\pcv x}{M\in\pcv x}\\[-6pt]
\downline
\end{array}
$$
\caption{Pseudo $x$-covalues}
\label{fig:pseudocv}
\end{figure}

\begin{figure}[!h]
$$
\begin{array}{|c|}
\upline\\[-6pt]
\infer{\cst V\in\pv}{\strut}
\qquad
\infer{\JCrx V y M\in\pv}{M\in\pv}\\[-6pt]
\downline
\end{array}
$$
\caption{Pseudo values}
\label{fig:pseudov}
\end{figure}

\begin{remark}\label{rem:stblred}
$\pv$ and $\pcv x$ are stable under reduction.
\end{remark}

\begin{remark}\label{rem:pcvnotpp}
In the next section we use the fact $\pv\cap\pcv x=\emptyset$ and its
immediate corollary that pseudo-principal cuts cannot be in $\pcv x$
(nor of course in $\pv$).
\end{remark}



\begin{definition}
\begin{itemize}
\item
We give in Fig.~\ref{fig:LJQl} an encoding of \lLJQ\ into the $\l$-calculus.
\begin{figure}[!h]
$$
\begin{array}{|lll|}
\upline
\ql x&\eqdef x&\\
\ql {\l x.M}&\eqdef \id\ \l x.\ql M&\\
\ql {\JCrxV V x {V'}}&\eqdef\subst{\ql {V'}}x{\ql V}&
\midline
\ql {\cst V}&\eqdef \ql V&\\
\ql {\ap x V y M}&\eqdef(\l y.\ql{M})\ (x\ {\ql V})&\\
\ql {\letin N x M}&\eqdef \subst{\ql {M}}x{\ql N}&N\in\pv\wedge
M\in\pcv x\\
\ql {\letin N x M}&\eqdef (\l x.\ql M)\ (\ql N)&\mbox{otherwise}\\
\ql {\JCrx V x M}&\eqdef\subst{\ql {M}}x{\ql V}&
\downline
\end{array}
$$
\caption{From \lLJQ\ to $\l$-calculus}
\label{fig:LJQl}
\end{figure}
\item
We define in \lLJQ\ the set of $\b$-\emph{bounded} terms (and values) as\\
$\bounded\eqdef
\{M\in\lLJQm\sep \forall N\subtermeq M, \ql N\in\SN\beta
\wedge \forall V'\subtermeq M, \ql {V'}\in\SN\beta{}\}\\
\strut\qquad\cup
\{V\in\lLJQm\sep \forall N\subtermeq V, \ql N\in\SN\beta
\wedge \forall V'\subtermeq V, \ql V'\in\SN\beta{}\}$
\end{itemize}
\end{definition}


\begin{remark}
\begin{itemize}
\item
$\FV{\ql M}\subseteq\FV{M}$
\item
$\ql{\subst M x y}=\subst {\ql M} x y$
\end{itemize}
\end{remark}

\begin{remark}\label{rem:worstcase}
$(\l x.\ql M)\ \ql N\Rewn{\sigm\b}\ql {\letin N x
  M}\Rewn{\sigm\b}\subst{\ql M}x{\ql N}$
\end{remark}

\begin{theorem}\label{th:simulat}
If $M\in\bounded$ (\resp $V\in\bounded$) and $M\Rew{\lLJQm}N$ (\resp
$V\Rew{\lLJQm}V'$), then $N\in\bounded$ (\resp $V'\in\bounded$) and
$\ql M\Rewn{\sigm\b} \ql N$ (\resp
$\ql V\Rewn{\sigm\b} \ql{V'}$).
\end{theorem}
\begin{proof}
By induction on the reduction steps $M\Rew{\lLJQm}N$ (\resp
$V\Rew{\lLJQm}V'$).  The following table gives the base case of the
induction: for each reduction rule, the left-hand side shows a term to
which $\ql M$ (\resp $\ql V$) $\sigm\b$-reduces (by
Remark~\ref{rem:worstcase}), while the right-hand side shows a term
that $\sigm\b$-reduces (by Remark~\ref{rem:worstcase}) to $\ql N$
(\resp $\ql {V'}$).
$$\begin{array}{|llll|}
\upline
&
(\l z.\ql P)\ (\id\ (\l x.\ql M)\ \ql V)\ &\Rewn{\sigm\b}
(\l z.\ql P)\ ((\l x.\ql M)\ \ql V)&\\
&       \subst {\ql N} y x&\Rewn{\sigm\b}\subst {\ql N} y x&\\
&       \subst y y {\ql M}&\Rewn{\sigm\b}\ql M&
\downline
\end{array}
$$

$$\begin{array}{|lll|}
\upline
        & (\l x.\ql N)\ ((\l y.\ql P)\ (z\ \ql V))&\Rewn{\sigm\b}(\l y.(\l x.\ql N)\ \ql P)\ (z\ \ql V)\\
        &(\l x.N)\ ((\l z.\ql P)\ (\ql {V'}\ \ql V))&\Rewn{\sigm\b}
(\l z.(\l x.\ql N)\ \ql P)\ (\ql {V'}\ \ql V)\\
        &(\l x.\ql N)\ (\subst{\ql P}y{\ql
          M})&\Rewn{\sigm\b}\subst{((\l x.\ql N)\ \ql P)}y{\ql
          M}\quad\mbox{ if $\letin M y P$ is pseudo principal}\\
&&\flush\mbox{(and thus $\letin M y {\letin N x P}$ is
          pseudo principal)}\\
        &(\l x.\ql N)\ ((\l y. \ql P)\ \ql M)&\Rewn{\sigm\b}(\l
        y.(\l x.\ql N)\ \ql P)\ \ql M\quad\mbox{ if not}\\
        &\subst{\ql N} x {\id\ \l y.\ql M}&\Rewn{\sigm\b}\subst{\ql N} x {\id\ \l y.\ql M}
\downline
\end{array}
$$

$$\begin{array}{|lll|}
\upline
&\subst x x {\ql V}&\Rewn{\sigm\b} \ql V\\
&\subst y x {\ql V}&\Rewn{\sigm\b} y\\
&\subst {(\id\ \l y.\ql M)} x {\ql V}&\Rewn{\sigm\b}\id\ \l y.\subst {\ql M} x {\ql V}
\midline
&\subst {\ql {V'}} x {\ql V}&\Rewn{\sigm\b}\subst {\ql {V'}} x {\ql V}\\
&\subst {((\l z.\ql P)\ (x\ \ql{V'}))} x {\ql V}&\Rewn{\sigm\b}
(\l z.\subst {\ql P} x {\ql V})\ ({\ql V}\ \subst {\ql{V'}} x {\ql V})\\
&\subst {((\l z.\ql P)\ (x'\ \ql{V'}))} x {\ql V}&\Rewn{\sigm\b}
(\l z.\subst {\ql P} x {\ql V})\ (x'\ \subst {\ql{V'}} x {\ql V})\\
&\subst{\subst{\ql P} y {\ql M}} x{\ql
  V}&\Rewn{\sigm\b}\subst{\subst{\ql P} x{\ql V}} y {\subst{\ql M} x{\ql V}}\quad\mbox{ if $\letin M y P$ is
          pseudo principal}\\
&&\flush\mbox{(and thus $\letin {\JCrx V x M} y {\JCrx V x P}$ is  pseudo principal)}\\
&\subst{((\l y.\ql P)\ \ql M)} x{\ql V}&\Rewn{\sigm\b}(\l y.\subst{\ql P} x{\ql V})\ \subst{\ql M} x{\ql V}\quad\mbox{ if not}\\
\hline
\end{array}
$$

The rest of the induction is straightforward, since $\Rew{\sigm\b}$ is
context-closed and principal cuts are stable under reduction
(Remark~\ref{rem:stblred}).
\end{proof}

\subsection{A labelled \LPO}

\begin{definition}
We define a first-order syntax by giving the following infinite signature:
$$\{\blob/0,\unname/1,\deuxname/2,\subiname[M]/2,\subiiname[M]/2,\subiiiname[M]/2,\subivname[M]/2\}$$
with $M$ ranging over the set of $\l$-terms in $\SN{\b}$.

We give them the following (terminating\footnote{because of Theorem~\ref{th:sbb}}) precedence:
$$\blob\pre\unname\pre\deuxname\pre\subiname[N]\pre\subiiname[N]\pre\subiiiname[N]\pre\subivname[N]\pre\subiname[M]$$
for all $M,N\in\SN{\sigm\b}$ such that $M(\Rew{\sigm\b}\cup\sustermeq)^*N$.

We now consider the (terminating) \emph{lexicographic path ordering}
induced by this precedence over first-order terms (see \eg \cite{Terese03}).
\end{definition}

We now want to encode $\b$-bounded \lLJQ-terms into this
first-order syntax to show that \lLJQ-reduction decreases first-order
encodings \wrt the \LPO.  For that we need to make a case distinction
to encode $\letin N x M$, as either a $\subiname$-construct or a
$\subiiiname$-one. Those to be encoded as a $\subiname$-construct are
identified as the set $\hpp$ defined in Fig.~\ref{fig:hpp}.
\begin{figure}[!h]
$$
\begin{array}{|c|}
\upline\\[-6pt]
\infer[x\not\in \FV V\cup\FV M]{\letin {\cst {V'}} x{\ap x V y M}\in\hpp}{}
\\\\
\infer[M\in\pcv x]{\JCrx V x M\in\hpp}{}
\qquad
\infer{\letin M x N\in\hpp}{M\in\hpp}\\
\downline
\end{array}
$$
\caption{Set of ``small'' cuts}
\label{fig:hpp}
\end{figure}


\begin{remark}\label{rem:hpppp}
Note that $\pv\cap\hpp=\emptyset$. Consequently, if $\letin M x
N\in\hpp$ is pseudo-principal, then it is principal.
\end{remark}

\begin{remark}\label{rem:Hppstblred}
$\hpp$ is stable under reduction.
\end{remark}

Fig.~\ref{fig:encfo} then gives the encoding into the first-order syntax.

\begin{figure}[!h]
$$
\begin{array}{|lll|}
\upline
\foc x&\eqdef \blob&\\
\foc {\l x.M}&\eqdef \un {\foc M}&\\
\foc {\JCrxV V x {V'}}&\eqdef\subiv[\ql{\JCrxV V x {V'}}]{\foc V}{\foc {V'}}&
\midline
\foc {\cst V}&\eqdef \un{\foc V}&\\
\foc {\ap x V y M}&\eqdef\deux{\foc V}{\foc{M}}&\\
\foc {\letin N x M}&\eqdef \subi[\ql{\letin N x M}]{\foc N}{\foc {M}}&\letin N x M\in\hpp\\
\foc {\letin N x M}&\eqdef \subiii[\ql{\letin N x M}]{\foc N}{\foc {M}}&\mbox{otherwise}\\
\foc {\JCrx V x M}&\eqdef \subii[\ql{\JCrx V x M}]{\foc V}{\foc {M}}&M\in\pcv x\\
\foc {\JCrx V x M}&\eqdef \subiv[\ql{\JCrx V x M}]{\foc V}{\foc {M}}&\mbox{otherwise}
\downline
\end{array}
$$
\caption{Encoding into the first-order syntax}
\label{fig:encfo}
\end{figure}

\begin{remark}
$\foc{\subst M y x}=\foc M$
\end{remark}

\begin{remark}\label{rem:worstcase2}\strut
\begin{enumerate}
\item
$\subiii[(\l x.\ql M)\ \ql{N}]{\foc N}{\foc M}\ (\glpo\cup=)\ \foc
{\letin N x M}\ (\glpo\cup=)\ \subi[\subst{\ql M} x{\ql{N}}]{\foc N}{\foc M}$
\item
$\subiv[\subst{\ql M} x{\ql{N}}]{\foc N}{\foc M}\ (\glpo\cup=)\ \foc
{\JCrx N x M}\ (\glpo\cup=)\ \subii[\subst{\ql M} x{\ql{N}}]{\foc N}{\foc M}$
\end{enumerate}
\end{remark}

\begin{theorem}
If $M\in\bounded$ (\resp $V\in\bounded$) and $M\Rew{\lLJQm}N$ (\resp
$V\Rew{\lLJQm}V'$), then $N\in\bounded$ (\resp $V'\in\bounded$) and
$\foc M\glpo \foc N$ (\resp
$\foc V\glpo \foc{V'}$).
\end{theorem}
\begin{proof}
By induction on the reduction steps $M\Rew{\lLJQm}N$ (\resp
$V\Rew{\lLJQm}V'$).  The following table gives the base case of the
induction: for each reduction rule, the left-hand side shows a term
that is (by Remarks~\ref{rem:worstcase} and~\ref{rem:worstcase2}) greater than or equal to $\foc
M$ (\resp $\foc V$), while the right-hand side shows a term that is
(by Remark~\ref{rem:worstcase} and~\ref{rem:worstcase2}) greater than or equal to $\foc N$
(\resp $\foc {V'}$).

$$
\begin{array}{|l@{\ }l|}
\upline
\subi[(\l z.\ql P)\ (\id\ (\l x.\ql M)\ \ql V)]{\un{\un{\foc
    M}}}{\deux{\foc V}{\foc P}}\flush&\glpo\ \subiii[(\l z.\ql P)\ ((\l
x.\ql M)\ \ql V)]{\subiii[(\l
x.\ql M)\ \ql V] {\un{\foc V}} {\foc M}} {\foc P}\\
\subiv[\subst {\ql N} y x]{\blob}{\foc
          N}\flush&\glpo\ \foc N\\
\subiv[\subst y y {\ql M}]{\foc
          M}\blob\flush&\glpo\ \foc M
\downline
\end{array}
$$

\begin{center}
\begin{tabular}{|l|}
\upline
\!\!$\begin{array}{l@{\ }l}
\subiii[(\l x.\ql N)\ ((\l y.\ql P)\ (z\ \ql
        V))]{\deux {\foc V}{\foc P}}{\foc N}&\glpo\   
\deux{\foc V}{\subiii[(\l y.(\l x.\ql N)\ \ql P)\ (z\ \ql V)]{\foc P}{\foc N}}\\
\subi[(\l x.\ql N)\ L]{\subi[L]{\un
            {V'}}{\deux{\foc V}{\foc P}}}{\foc N}
&\glpo\   \subi[(\l z.L')\ (\ql {V'}\ \ql V)]{\un{\foc
    {V'}}}{\subiii[L']{\foc P}{\foc N}}
\end{array}$\\
\flush with $L=(\l z.\ql P)\ (\ql {V'}\ \ql
          V)$ and $L'=(\l x.\ql N)\ \ql P$\\\\
The next rule splits into two cases:\footnotemark\\
\!\!$\begin{array}{l@{\ }l}
\subi[(\l x.\ql N)\ L]{\subi[L] {\foc M}{\foc P}}{\foc N}&\glpo\   
\subi[(\l y.L')\ \ql M]{\foc M} {\subiii[L']{\foc P}{\foc N}}
\quad \mbox{if $\letin M y P\in\hpp$}\\
      &       \hfill \mbox{with $L=(\l y.\ql P)\ {\ql M}$
          and $L'=(\l x.\ql N)\ \ql P$}\\&\\
\subiii[(\l x.\ql N)\ L]{\subiii[L] {\foc M}{\foc P}}{\foc N}&\glpo\   
\subiii[L']{\foc M} {\subiii[(\l x.\ql N)\ \ql P]{\foc P}{\foc N}}
\flush \mbox{if not, with,}
\end{array}$\\
\!\!\begin{tabular}{l@{\ }l@{\ }l}
if $\letin M y P$ is pseudo principal,&$L=\subst {\ql P} y{\ql M}$&and $L'=\subst{((\l x.\ql N)\ \ql P)}y{\ql
          M}$\\
otherwise&$L=(\l y.\ql P)\ {\ql M}$&and $L'=(\l
        y.(\l x.\ql N)\ \ql P)\ \ql M$
\end{tabular}\hspace{-13pt}\strut\\\\
The last rule, again, splits into two cases:\footnotemark\\
\!\!$\begin{array}{l@{\ }l}
\subiii[\subst{\ql N} x {\id\ \l y.\ql M}]{\un{\un{\foc M}}} {\foc N}&\glpo\   \subii[\subst{\ql N} x {\id\ \l y.\ql M}]{\un{\foc M}} {\foc N}
        \qquad\flush\mbox{ if $N\in\pcv x$}\\
\subiii[(\l x.{\ql N})\ {(\id\ \l y.\ql M)}]{\un{\un{\foc M}}} {\foc N}&\glpo\   \subiv[\subst{\ql N} x {\id\ \l y.\ql M}]{\un{\foc M}} {\foc N}
        \flush\mbox{ if not}
\end{array}$
\downline
\end{tabular}
\end{center}
\footnotetext[2]{Given the
condition (for the rule to apply) that $\letin M y P$ is not
principal, $\letin M y P\in\hpp$ \iff\ $M\in\hpp$ \iff\ $\letin M y
{\letin P x N}\in\hpp$ \iff\ $\letin {\letin M y P}x N\in\hpp$.
Moreover, in the first case, $\letin M y P\in\hpp$ entails
that it is not pseudo-principal (by Remark~\ref{rem:hpppp}), hence the
shape of $L$ (and note that $L\Rew{\sigm}(\l y.(\l x.\ql N)\ \ql P)\ \ql
M\susterm L'$).}
\footnotetext{In both cases of the last rule, we have encoded the redex as a
$\subiiiname$-construct since it is not principal and thus it cannot
be in $\hpp$.}

$$
\begin{array}{|l@{\ }l|}
\upline
\subiv[\ql V]{\foc V}\blob&\glpo\    \foc V\\
\subiv[y] {\foc V} \blob&\glpo\    \blob\\
\subiv[\subst{(\id\ \l y.\ql M)}x{\ql V}]{\foc V}{\un{\foc M}}
&\glpo\  \un{\subiv[\subst{\ql M}x{\ql V}]{\foc V}{\foc M}}
\midline
\subiv[\subst {\ql {V'}} x {\ql V}]{\foc V} {\un{\foc {V'}}}&\glpo\   \un {\subiv[\subst {\ql {V'}} x {\ql V}] {\foc V} {\foc {V'}}}\\&\\
\subii[L]{\foc V}
{\deux{\foc {V'}}{\foc P}}&\glpo\   
\subi[L]{\un{\foc V}}{\deux{\subiv[\subst {\ql{V'}} x
{\ql V}]{\foc V}{\foc {V'}}}{\subiv[\subst {\ql{P}} x
{\ql V}]{\foc V}{\foc P}}}\\
&\flush\mbox{with $L=\subst {((\l z.\ql P)\ (x\ \ql{V'}))} x {\ql V}$}\\&\\
\subiv[L]{\foc V} {\deux{\foc {V'}}{\foc P}}&\glpo\   \deux{\subiv[\subst {\ql{V'}} x
{\ql V}]{\foc V}{\foc {V'}}}{\subiv[\subst {\ql{P}} x
{\ql V}]{\foc V}{\foc P}}\\
&\flush\mbox{with $L=\subst {((\l z.\ql P)\ (x'\ \ql{V'}))} x {\ql V}$}\\
\mbox{The last rule splits into two cases:\footnotemark}\hspace{-50pt}&\\
\subii[\subst{L} x{\ql V}]{\foc V} {\subi[L]{\foc M}{\foc P}}&
\glpo\   \subi[\subst{L} x{\ql V}]{\subii[L_M]{\foc V}{\foc M}}{\subiv[L_P]{\foc V}{\foc P}}
\quad\mbox{if }\letin M y P\in\pcv x\\&\\
&\flush\mbox{with $L=(\l y.\ql P)\ \ql M$, $L_M=\subst{\ql M} x{\ql V}$, and $L_P=\subst{\ql P} x{\ql V}$}\\
\subiv[\subst{L} x{\ql V}]{\foc V} {\subi[L]{\foc M}{\foc P}}&
\glpo\   \subiii[\subst{L} x{\ql V}]{\subiv[L_M]{\foc V}{\foc M}}{\subiv[L_P]{\foc V}{\foc P}}
\flush\mbox{if not}\\&\\
\flush\mbox{with $L=(\l y.\ql P)\ \ql M$}
&\!\mbox{or $L=\subst {\ql P}y{\ql M}$, $L_M=\subst{\ql M} x{\ql V}$, and $L_P=\subst{\ql P} x{\ql V}$}
\downline
\end{array}
$$\footnotetext{If $\letin M y P\in\pcv x$, first it cannot be pseudo
principal (Remark~\ref{rem:pcvnotpp}), and second we also have
$M\in\pcv x$ so $\letin {\JCrx V x M} y {\JCrx V x P}\in\hpp$. Also
note that $L_P\subterm \subst{L} x{\ql V}$.}

The inductive argument is straightforward, given that
$\pcv x$ and $\hpp$ are stable under reduction and the fact that, by
Theorem~\ref{th:simulat}, internal reductions can only decrease labels
with respect to $(\Rew{\sigm\b}\cup\susterm)$.
\end{proof}

\begin{corollary}\label{cor:yahoo}
$\bounded\subseteq\SN{}$
\end{corollary}
\begin{proof}
By Theorem~\ref{Th:SNbySimul}: the decreasing and terminating \LPO\
simulates \lLJQ-reductions through $\foc{(\ \cdot\ )}$\ . 
\end{proof}

\subsection{Conclusion}
\begin{lemma}\label{lem:typpreserved}
If $\Deri \Gamma M A$ then, for every $N\subtermeq M$ (\resp $V\subtermeq
M$), $\Deri[\lambda] \Gamma {\ql M} A$ (\resp $\Deri[\lambda] \Gamma  {\ql V} A$) in
the simply-typed $\l$-calculus.
\end{lemma}
\begin{proof}
Straightforward induction on the typing tree, using the typing property
of substitution in $\l$-calculus.
\end{proof}

\begin{theorem}
If $\Deri \Gamma M A$ then $M\in\SN{}$.
\end{theorem}
\begin{proof}
By Lemma~\ref{lem:typpreserved} and the strong normalisation of the
simply-typed $\l$-calculus, $M\in\bounded$ so $M\in\SN{}$ by
Corollary~\ref{cor:yahoo}.
\end{proof}

==> LJQ.tex <==
\section{\lLJQ}

\begin{definition}[\lLJQ]
\begin{itemize}
\item
The syntax of \lLJQ\ comes as two syntactic categories, the first one
of which being that of \emph{values}:
$$
\begin{array}{lll}
V, V' & ::=     & x        
        \sep    \l x.M                        
        \sep    \JCrxV{V}{x}{V'}
\\
M,N,P & ::=     & \cst{V}       
                        \sep   \ap{x}{V}{y}{N} 
                        \sep    \JCrx{V}{x}{N}
                        \sep   \letin{M}{x}{N}
\end{array}
$$
\item
We define {\emph{$x$-covalues}} as those terms of the form $\cst x$ or $\ap
x V y M$ with $x\not\in\FV V\cup\FV M$.
\item
We define {\emph{principal cuts}} as those terms of the form
$\letin {\cst V} x M$ where $M$ is an $x$-covalue.
\item
The typing rules are shown in Fig.~\ref{Fig:LJQterms}. Derivability,
in the typing system of \lLJQ, of the sequents $\Deriv{\Gamma} V A$
and $\Deri{\Gamma} M A$, is denoted $\DeriLJQv{\Gamma} V A$ and
$\DeriLJQ{\Gamma} M A$, respectively.
\begin{figure}[!h]
{\small
$$
\begin{array}{|cc|}
\hline&\\
\infers{\strut}{\Deriv{\Gamma,x\col A} x A}{}&\quad \infers {\Deriv
  {\Gamma} V A}
{\Deri \Gamma {\cst V} A}{}\\
&\\
\infers{\Deri {\Gamma,x\col A} M B}{\Deriv \Gamma{\l x.M}{A\arr B}}{}
&\quad
\infers{\Deriv {\Gamma,x\col A\arr B} V {A}\quad \Deri {\Gamma,x\col
    A\arr B,y\col B} N C}{\Deri
{\Gamma,x\col A\arr B} {\ap x V y N} C}{}\\
&\\
\infers {\Deriv \Gamma V A\quad
\Deriv {\Gamma,x\col A} {V'} B}{\Deriv \Gamma {\JCrxV{V}{x}{V'}} B}{}
&\quad \infers {\Deriv \Gamma V A\quad
\Deri {\Gamma,x\col A} N B}{\Deri \Gamma {\JCrxV{V}{x}{N}} B}{}\\
&\\
&\quad \infers {\Deri \Gamma M A\quad
\Deri {\Gamma,x\col A} N B}{\Deri \Gamma {\letin M x N} B}{}\\
&\\
\hline
\end{array}
$$}
\caption{Typing system of \lLJQ}
\label{Fig:LJQterms}
\end{figure}
\item
The reduction system, also called $\lLJQm$, is shown in Fig.~\ref{Fig:LJQredbis}.
\begin{figure}[!h]
$$
\begin{array}{|lll|}
\upline
&\flush
\letin{\cst{\l x.M}}y{\ap y V z P}\flush&\Rew{}\letin {\letin {\cst V} x M} z
P\quad\mbox{if
$y\notin \FV V\cup \FV P$}\\
        &\flush       \letin {\cst x} y N\flush&\Rew{}\subst N  y x\\
        &\flush       \letin M y {\cst y}\flush&\Rew{}M
\mmidline
        &\flush\letin {\ap z V y P} x N&\Rew{}\ap z V y {\letin  P x N}\\
        &\flush\letin {\letin {\cst {V'}} y {\ap y V z P}} x N&\Rew{}\letin{\cst {V'}} y {\ap y V z {\letin  P x N}}\\
        &       &\hfill\mbox{if $y\notin \FV V\cup \FV P$}\\
        &\flush\letin {\letin M y P} x N&\Rew{}\letin M y {\letin  P x N}\\
        &       &       \hfill \mbox{if the redex is not one of the
previous rule}\\
        &\flush\letin {\cst {\l y.M}} x N&\Rew{}\JCrx {\lambda y.M} x N
        \mbox{ if $N$ is not an $x$-covalue}
\mmidline
&\JCrxV V x x&\Rew{} V\\
&\JCrxV V x y&\Rew{} y\\
&\JCrxV V x {\l y.M}&\Rew{}{\l y.\JCrx V x M}
\midline
&\JCrx V x {\cst {V'}}&\Rew{}\cst {\JCrxV V x {V'}}\\
&\JCrx V x {\ap x {V'} z P}&\Rew{}\letin {\cst V} x {\ap x {\JCrxV V x {V'}} z {\JCrx
V x P}}\\
&\JCrx V x {\ap {x'} {V'} z P}&\Rew{}{\ap {x'} {\JCrxV {V} x {V'}} z {\JCrx V x P}}\\
&\JCrx V x {\letin M y P}&\Rew{}\letin {\JCrx V x M} y {\JCrx V x P}
\downline
\end{array}
$$
\caption{Reduction rules of \lLJQ}
\label{Fig:LJQredbis}
\end{figure}
\end{itemize}
\end{definition}

As mentioned earlier, the purpose of this paper is to prove that if $\Deri \Gamma M A$ then $M\in\SN{}$.

\section{Strong normalisation of \lLJQ}
\subsection{An encoding into $\l$-calculus}

\begin{definition}
In Fig.~\ref{fig:pseudov} and Fig.~\ref{fig:pseudocv}, we inductively
define the set $\pv$ of \emph{pseudo values} and the set $\pcv x$ of
\emph{pseudo $x$-covalues}, respectively. A cut $\letin N x M$ is said
to be \emph{pseudo principal} if $N\in\pv$ and $M\in\pcv x$.
\end{definition}


\begin{remark}\label{rem:pcvnotpp}
Note that $\pv\cap\pcv x=\emptyset$ and its
immediate corollary that pseudo principal cuts cannot be in $\pcv x$
(nor of course in $\pv$).
\end{remark}

\begin{remark}\label{rem:stblred}
$\pv$ and $\pcv x$ are stable under reduction.
\end{remark}

\begin{remark}\label{rem:stblsub} Suppose $x\neq y$ and $x\neq z$.
If $M$ is in $\pcv x$ (\resp in $\pv$) then so is $\subst M y
z$. Hence if $M$ is a pseudo principal cut then so is $\subst M y z$.
\end{remark}

\begin{figure}[!t]
$$
\begin{array}{|c|}
\upline\\[-6pt]
\infer{\cst V\in\pv}{\strut}
\qquad
\infer{\JCrx V y M\in\pv}{M\in\pv}\\[-6pt]
\downline
\end{array}
$$
\caption{Pseudo values}
\label{fig:pseudov}
\end{figure}

\begin{figure}[t]
$$
\begin{array}{|c|}
\upline\\[-6pt]
\infer[x\not\in \FV V\cup\FV M]{\ap x V y M\in\pcv x}{}
\\\\
\infer[x\not\in \FV V]{\JCrx V y M\in\pcv x}{M\in\pcv x}
\qquad
\infer[x\not\in \FV N]{\letin M y N\in\pcv x}{M\in\pcv x}\\[-6pt]
\downline
\end{array}
$$
\caption{Pseudo $x$-covalues}
\label{fig:pseudocv}
\end{figure}


\begin{definition}
\begin{itemize}
\item
We give in Fig.~\ref{fig:LJQl} an encoding of \lLJQ\ into the $\l$-calculus.
\begin{figure}[!h]
$$
\begin{array}{|lll|}
\upline
\ql x&\eqdef x&\\
\ql {\l x.M}&\eqdef \id\ \l x.\ql M&\\
\ql {\JCrxV V x {V'}}&\eqdef\subst{\ql {V'}}x{\ql V}&
\midline
\ql {\cst V}&\eqdef \ql V&\\
\ql {\ap x V y M}&\eqdef(\l y.\ql{M})\ (x\ {\ql V})&\\
\ql {\letin N x M}&\eqdef \subst{\ql {M}}x{\ql N}&N\in\pv\wedge
M\in\pcv x\\
\ql {\letin N x M}&\eqdef (\l x.\ql M)\ (\ql N)&\mbox{otherwise}\\
\ql {\JCrx V x M}&\eqdef\subst{\ql {M}}x{\ql V}&
\downline
\end{array}
$$
\caption{From \lLJQ\ to $\l$-calculus}
\label{fig:LJQl}
\end{figure}
\item
We define in \lLJQ\ the set of $\b$-\emph{bounded} terms (and values) as\\
$\bounded\eqdef
\{M\in\lLJQm\sep \forall N\subtermeq M, \ql N\in\SN\beta
\wedge \forall V'\subtermeq M, \ql {V'}\in\SN\beta{}\}\\
\strut\qquad\cup
\{V\in\lLJQm\sep \forall N\subtermeq V, \ql N\in\SN\beta
\wedge \forall V'\subtermeq V, \ql V'\in\SN\beta{}\}$
\end{itemize}
\end{definition}


\begin{remark}Note that
$\FV{\ql M}\subseteq\FV{M}$ and, from Remark~\ref{rem:stblsub},
$\ql{\subst M x y}=\subst {\ql M} x y$.
\end{remark}

\begin{remark}\label{rem:worstcase}
$(\l x.\ql M)\ \ql N\Rewn{\sigm\b}\ql {\letin N x
  M}\Rewn{\sigm\b}\subst{\ql M}x{\ql N}$
\end{remark}

\begin{theorem}\label{th:simulat}
If $M\in\bounded$ (\resp $V\in\bounded$) and $M\Rew{\lLJQm}N$ (\resp
$V\Rew{\lLJQm}V'$), then $N\in\bounded$ (\resp $V'\in\bounded$) and
$\ql M\Rewn{\sigm\b} \ql N$ (\resp
$\ql V\Rewn{\sigm\b} \ql{V'}$).
\end{theorem}
\begin{proof}
By induction on the reduction steps $M\Rew{\lLJQm}N$ (\resp
$V\Rew{\lLJQm}V'$).  The following table gives the base case of the
induction: for each reduction rule, the left-hand side shows a term to
which $\ql M$ (\resp $\ql V$) $\sigm\b$-reduces (by
Remark~\ref{rem:worstcase}), while the right-hand side shows a term
that $\sigm\b$-reduces (by Remark~\ref{rem:worstcase}) to $\ql N$
(\resp $\ql {V'}$).

$$\begin{array}{|llll|}
\upline
&
(\l z.\ql P)\ (\id\ (\l x.\ql M)\ \ql V)\ &\Rewn{\sigm\b}
(\l z.\ql P)\ ((\l x.\ql M)\ \ql V)&\\
&       \subst {\ql N} y x&\Rewn{\sigm\b}\subst {\ql N} y x&\\
&       \subst y y {\ql M}&\Rewn{\sigm\b}\ql M&
\downline
\end{array}
$$

$$\begin{array}{|lll|}
\upline
        & (\l x.\ql N)\ ((\l y.\ql P)\ (z\ \ql V))&\Rewn{\sigm\b}(\l y.(\l x.\ql N)\ \ql P)\ (z\ \ql V)\\
        &(\l x.N)\ ((\l z.\ql P)\ (\ql {V'}\ \ql V))&\Rewn{\sigm\b}
(\l z.(\l x.\ql N)\ \ql P)\ (\ql {V'}\ \ql V)\\
        &(\l x.\ql N)\ (\subst{\ql P}y{\ql
          M})&\Rewn{\sigm\b}\subst{((\l x.\ql N)\ \ql P)}y{\ql
          M}\quad\mbox{ if $\letin M y P$ is pseudo principal}\\
&&\flush\mbox{(and thus $\letin M y {\letin P x N}$ is
          pseudo principal)}\\
        &(\l x.\ql N)\ ((\l y. \ql P)\ \ql M)&\Rewn{\sigm\b}(\l
        y.(\l x.\ql N)\ \ql P)\ \ql M\quad\mbox{ if not}\\
        &\subst{\ql N} x {\id\ \l y.\ql M}&\Rewn{\sigm\b}\subst{\ql N} x {\id\ \l y.\ql M}
\downline
\end{array}
$$

$$\begin{array}{|lll|}
\upline
&\subst x x {\ql V}&\Rewn{\sigm\b} \ql V\\
&\subst y x {\ql V}&\Rewn{\sigm\b} y\\
&\subst {(\id\ \l y.\ql M)} x {\ql V}&\Rewn{\sigm\b}\id\ \l y.\subst {\ql M} x {\ql V}
\midline
&\subst {\ql {V'}} x {\ql V}&\Rewn{\sigm\b}\subst {\ql {V'}} x {\ql V}\\
&\subst {((\l z.\ql P)\ (x\ \ql{V'}))} x {\ql V}&\Rewn{\sigm\b}
(\l z.\subst {\ql P} x {\ql V})\ ({\ql V}\ \subst {\ql{V'}} x {\ql V})\\
&\subst {((\l z.\ql P)\ (x'\ \ql{V'}))} x {\ql V}&\Rewn{\sigm\b}
(\l z.\subst {\ql P} x {\ql V})\ (x'\ \subst {\ql{V'}} x {\ql V})\\
&\subst{\subst{\ql P} y {\ql M}} x{\ql
  V}&\Rewn{\sigm\b}\subst{\subst{\ql P} x{\ql V}} y {\subst{\ql M} x{\ql V}}\quad\mbox{ if $\letin M y P$ is
          pseudo principal}\\
&&\flush\mbox{(and thus $\letin {\JCrx V x M} y {\JCrx V x P}$ is  pseudo principal)}\\
&\subst{((\l y.\ql P)\ \ql M)} x{\ql V}&\Rewn{\sigm\b}(\l y.\subst{\ql P} x{\ql V})\ \subst{\ql M} x{\ql V}\quad\mbox{ if not}\\
\hline
\end{array}
$$

The rest of the induction is straightforward, since $\Rew{\sigm\b}$ is
context-closed and principal cuts are stable under reduction
(Remark~\ref{rem:stblred}).
\end{proof}

\subsection{A labelled \LPO}

\begin{definition}
We define a first-order syntax by giving the following infinite signature:
$$\{\blob/0,\unname/1,\deuxname/2,\subiname[M]/2,\subiiname[M]/2,\subiiiname[M]/2,\subivname[M]/2\}$$
with $M$ ranging over the set of $\l$-terms in $\SN{\b}$.

We give them the following (terminating\footnote{because of Theorem~\ref{th:sbb}}) precedence:
$$\blob\pre\unname\pre\deuxname\pre\subiname[N]\pre\subiiname[N]\pre\subiiiname[N]\pre\subivname[N]\pre\subiname[M]$$
for all $M,N\in\SN{\sigm\b}$ such that $M(\Rew{\sigm\b}\cup\sustermeq)^*N$.

We now consider the (terminating) \emph{lexicographic path ordering}
induced by this precedence over first-order terms (see \eg \cite{Terese03}).
\end{definition}

We now want to encode $\b$-bounded \lLJQ-terms into this
first-order syntax to show that \lLJQ-reduction decreases first-order
encodings \wrt the \LPO.  For that we need to make a case distinction
to encode $\letin N x M$, as either a $\subiname$-construct or a
$\subiiiname$-one. Those to be encoded as a $\subiname$-construct are
identified as the set $\hpp$ defined in Fig.~\ref{fig:hpp}.
\begin{figure}[!h]
$$
\begin{array}{|c|}
\upline\\[-6pt]
\infer[x\not\in \FV V\cup\FV M]{\letin {\cst {V'}} x{\ap x V y M}\in\hpp}{}
\\\\
\infer[M\in\pcv x]{\JCrx V x M\in\hpp}{}
\qquad
\infer{\letin M x N\in\hpp}{M\in\hpp}\\
\downline
\end{array}
$$
\caption{Set of ``small'' cuts}
\label{fig:hpp}
\end{figure}


\begin{remark}\label{rem:hpppp}
Note that $\pv\cap\hpp=\emptyset$. Consequently, if $\letin {M}
x{N}\in\hpp$ with $M\in\pv$, then it is of the form $\letin {\cst
V}x{\ap x {V'} y P}$ with $x\not\in \FV V\cup\FV P$.
\end{remark}

\begin{remark}\label{rem:Hppstblred}
If $M\Rewn{}M'$, $N\Rewn{}N'$, $V\Rewn{}V'$ and $\letin M x N$ (\resp
$\JCrx V x N$) is in $\hpp$, then so is $\letin {M'} x {N'}$ (\resp
$\JCrx {V'} x {N'}$).
\end{remark}

\begin{remark}\label{rem:stblsub2} If $M$ is in  $\hpp$ then so is
  $\subst M y z$.
\end{remark}

Fig.~\ref{fig:encfo} then gives the encoding into the first-order
syntax.

\begin{figure}[!h]
$$
\begin{array}{|lll|}
\upline
\foc x&\eqdef \blob&\\
\foc {\l x.M}&\eqdef \un {\foc M}&\\
\foc {\JCrxV V x {V'}}&\eqdef\subiv[\ql{\JCrxV V x {V'}}]{\foc V}{\foc {V'}}&
\midline
\foc {\cst V}&\eqdef \un{\foc V}&\\
\foc {\ap x V y M}&\eqdef\deux{\foc V}{\foc{M}}&\\
\foc {\letin N x M}&\eqdef \subi[\ql{\letin N x M}]{\foc N}{\foc {M}}&\letin N x M\in\hpp\\
\foc {\letin N x M}&\eqdef \subiii[\ql{\letin N x M}]{\foc N}{\foc {M}}&\mbox{otherwise}\\
\foc {\JCrx V x M}&\eqdef \subii[\ql{\JCrx V x M}]{\foc V}{\foc {M}}&\JCrx V x M\in\hpp\\
\foc {\JCrx V x M}&\eqdef \subiv[\ql{\JCrx V x M}]{\foc V}{\foc {M}}&\mbox{otherwise}
\downline
\end{array}
$$
\caption{Encoding into the first-order syntax}
\label{fig:encfo}
\end{figure}

\begin{remark}By Remark~\ref{rem:stblsub2},
$\foc{\subst M y x}=\foc M$.
\end{remark}

\begin{remark}\label{rem:worstcase2}\strut
\begin{enumerate}
\item
$\subiii[(\l x.\ql M)\ \ql{N}]{\foc N}{\foc M}\ (\glpo\cup=)\ \foc
{\letin N x M}\ (\glpo\cup=)\ \subi[\subst{\ql M} x{\ql{N}}]{\foc N}{\foc M}$
\item
$\subiv[\subst{\ql M} x{\ql{N}}]{\foc N}{\foc M}\ (\glpo\cup=)\ \foc
{\JCrx N x M}\ (\glpo\cup=)\ \subii[\subst{\ql M} x{\ql{N}}]{\foc N}{\foc M}$
\end{enumerate}
\end{remark}

\begin{theorem}
If $M\in\bounded$ (\resp $V\in\bounded$) and $M\Rew{\lLJQm}N$ (\resp
$V\Rew{\lLJQm}V'$), then $N\in\bounded$ (\resp $V'\in\bounded$) and
$\foc M\glpo \foc N$ (\resp
$\foc V\glpo \foc{V'}$).
\end{theorem}
\begin{proof}
By induction on the reduction steps $M\Rew{\lLJQm}N$ (\resp
$V\Rew{\lLJQm}V'$).  The following table gives the base case of the
induction: for each reduction rule, the left-hand side shows a term
that is (by Remarks~\ref{rem:worstcase} and~\ref{rem:worstcase2})
greater than or equal to $\foc M$ (\resp $\foc V$), while the
right-hand side shows a term that is (by Remark~\ref{rem:worstcase}
and~\ref{rem:worstcase2}) greater than or equal to $\foc N$ (\resp
$\foc {V'}$).

$$
\begin{array}{|l@{\ }l|}
\upline
\subi[(\l z.\ql P)\ (\id\ (\l x.\ql M)\ \ql V)]{\un{\un{\foc
    M}}}{\deux{\foc V}{\foc P}}\flush&\glpo\ \subiii[(\l z.\ql P)\ ((\l
x.\ql M)\ \ql V)]{\subiii[(\l
x.\ql M)\ \ql V] {\un{\foc V}} {\foc M}} {\foc P}\\
\subiv[\subst {\ql N} y x]{\blob}{\foc
          N}\flush&\glpo\ \foc N\\
\subiv[\subst y y {\ql M}]{\foc
          M}\blob\flush&\glpo\ \foc M
\downline
\end{array}
$$

\begin{center}
\begin{tabular}{|l|}
\upline
\!\!$\begin{array}{l@{\ }l}
\subiii[(\l x.\ql N)\ ((\l y.\ql P)\ (z\ \ql
        V))]{\deux {\foc V}{\foc P}}{\foc N}&\glpo\   
\deux{\foc V}{\subiii[(\l y.(\l x.\ql N)\ \ql P)\ (z\ \ql V)]{\foc P}{\foc N}}\\
\subi[(\l x.\ql N)\ L]{\subi[L]{\un
            {V'}}{\deux{\foc V}{\foc P}}}{\foc N}
&\glpo\   \subi[(\l z.L')\ (\ql {V'}\ \ql V)]{\un{\foc
    {V'}}}{\subiii[L']{\foc P}{\foc N}}
\end{array}$\\
\flush with $L=(\l z.\ql P)\ (\ql {V'}\ \ql
          V)$ and $L'=(\l x.\ql N)\ \ql P$\\\\
The next rule splits into two cases:\footnotemark\\
\!\!$\begin{array}{l@{\ }l}
\subi[(\l x.\ql N)\ L]{\subi[L] {\foc M}{\foc P}}{\foc N}&\glpo\   
\subi[(\l y.L')\ \ql M]{\foc M} {\subiii[L']{\foc P}{\foc N}}
\quad \mbox{if $\letin M y P\in\hpp$}\\
      &       \hfill \mbox{with $L=(\l y.\ql P)\ {\ql M}$
          and $L'=(\l x.\ql N)\ \ql P$}\\&\\
\subiii[(\l x.\ql N)\ L]{\subiii[L] {\foc M}{\foc P}}{\foc N}&\glpo\   
\subiii[L']{\foc M} {\subiii[(\l x.\ql N)\ \ql P]{\foc P}{\foc N}}
\flush \mbox{if not, with,}
\end{array}$\\
\!\!\begin{tabular}{l@{\ }l@{\ }l}
if $\letin M y P$ is pseudo principal,&$L=\subst {\ql P} y{\ql M}$&and $L'=\subst{((\l x.\ql N)\ \ql P)}y{\ql
          M}$\\
otherwise&$L=(\l y.\ql P)\ {\ql M}$&and $L'=(\l
        y.(\l x.\ql N)\ \ql P)\ \ql M$
\end{tabular}\hspace{-13pt}\strut\\\\
The last rule, again, splits into two cases:\footnotemark\\
\!\!$\begin{array}{l@{\ }l}
\subiii[\subst{\ql N} x {\id\ \l y.\ql M}]{\un{\un{\foc M}}} {\foc N}&\glpo\   \subii[\subst{\ql N} x {\id\ \l y.\ql M}]{\un{\foc M}} {\foc N}
        \qquad\flush\mbox{ if $N\in\pcv x$}\\
\subiii[(\l x.{\ql N})\ {(\id\ \l y.\ql M)}]{\un{\un{\foc M}}} {\foc N}&\glpo\   \subiv[\subst{\ql N} x {\id\ \l y.\ql M}]{\un{\foc M}} {\foc N}
        \flush\mbox{ if not}
\end{array}$
\downline
\end{tabular}
\end{center}
\footnotetext[2]{Given the condition on $\letin M y P$ for the rule to
apply, $\letin M y P\in\hpp$ \iff\ $M\in\hpp$ \iff\ $\letin M y
{\letin P x N}\in\hpp$ \iff\ $\letin {\letin M y P}x N\in\hpp$.
Moreover, in the first case, $\letin M y P\in\hpp$ entails that it is
not pseudo principal (by Remark~\ref{rem:hpppp}), hence the shape of
$L$ (and note that $L\Rew{\sigm}(\l y.(\l x.\ql N)\ \ql P)\ \ql
M\susterm L'$).}  \footnotetext{In both cases of the last rule, we
have encoded the redex as a $\subiiiname$-construct since it cannot be
in $\hpp$ (by Remark~\ref{rem:hpppp}).}

$$
\begin{array}{|l@{\ }l|}
\upline
\subiv[\ql V]{\foc V}\blob&\glpo\    \foc V\\
\subiv[y] {\foc V} \blob&\glpo\    \blob\\
\subiv[\subst{(\id\ \l y.\ql M)}x{\ql V}]{\foc V}{\un{\foc M}}
&\glpo\  \un{\subiv[\subst{\ql M}x{\ql V}]{\foc V}{\foc M}}
\midline
\subiv[\subst {\ql {V'}} x {\ql V}]{\foc V} {\un{\foc {V'}}}&\glpo\   \un {\subiv[\subst {\ql {V'}} x {\ql V}] {\foc V} {\foc {V'}}}\\
\subii[L]{\foc V}
{\deux{\foc {V'}}{\foc P}}&\glpo\   
\subi[L]{\un{\foc V}}{\deux{\subiv[\subst {\ql{V'}} x
{\ql V}]{\foc V}{\foc {V'}}}{\subiv[\subst {\ql{P}} x
{\ql V}]{\foc V}{\foc P}}}\\
&\flush\mbox{with $L=\subst {((\l z.\ql P)\ (x\ \ql{V'}))} x {\ql V}$}\\
\subiv[L]{\foc V} {\deux{\foc {V'}}{\foc P}}&\glpo\   \deux{\subiv[\subst {\ql{V'}} x
{\ql V}]{\foc V}{\foc {V'}}}{\subiv[\subst {\ql{P}} x
{\ql V}]{\foc V}{\foc P}}\\
&\flush\mbox{with $L=\subst {((\l z.\ql P)\ (x'\ \ql{V'}))} x {\ql V}$}\\
\mbox{The last rule splits into two cases:\footnotemark}\hspace{-50pt}&\\
\subii[\subst{L} x{\ql V}]{\foc V} {\subi[L]{\foc M}{\foc P}}&
\glpo\   \subi[\subst{L} x{\ql V}]{\subii[L_M]{\foc V}{\foc M}}{\subiv[L_P]{\foc V}{\foc P}}
\quad\mbox{if }\letin M y P\in\pcv x\\
&\flush\mbox{with $L=(\l y.\ql P)\ \ql M$, $L_M=\subst{\ql M} x{\ql V}$, and $L_P=\subst{\ql P} x{\ql V}$}\\
\subiv[\subst{L} x{\ql V}]{\foc V} {\subi[L]{\foc M}{\foc P}}&
\glpo\   \subiii[\subst{L} x{\ql V}]{\subiv[L_M]{\foc V}{\foc M}}{\subiv[L_P]{\foc V}{\foc P}}
\flush\mbox{if not}\\
\flush\mbox{with $L=(\l y.\ql P)\ \ql M$}
&\!\mbox{or $L=\subst {\ql P}y{\ql M}$, $L_M=\subst{\ql M} x{\ql V}$, and $L_P=\subst{\ql P} x{\ql V}$}
\downline
\end{array}
$$
\footnotetext{If $\letin M y P\in\pcv x$, first it cannot be pseudo
principal (Remark~\ref{rem:pcvnotpp}), and second we also have
$M\in\pcv x$ so $\letin {\JCrx V x M} y {\JCrx V x P}\in\hpp$. Also
note that $L_P\subterm \subst{L} x{\ql V}$.}

The inductive argument is straightforward, given that
$\pcv x$ and $\hpp$ are stable under reduction and the fact that, by
Theorem~\ref{th:simulat}, internal reductions can only decrease labels
with respect to $(\Rew{\sigm\b}\cup\susterm)$.
\end{proof}

\begin{corollary}\label{cor:yahoo}
$\bounded\subseteq\SN{}$
\end{corollary}
\begin{proof}
By Theorem~\ref{Th:SNbySimul}: the decreasing and terminating \LPO\
simulates \lLJQ-reductions through $\foc{(\ \cdot\ )}$\ . 
\end{proof}

\subsection{Conclusion}
\begin{lemma}\label{lem:typpreserved}
If $\Deri \Gamma M A$ then, for every $N\subtermeq M$ (\resp $V\subtermeq
M$), $\Deri[\lambda] \Gamma {\ql M} A$ (\resp $\Deri[\lambda] \Gamma  {\ql V} A$) in
the simply-typed $\l$-calculus.
\end{lemma}
\begin{proof}
Straightforward induction on the typing tree, using the typing property
of substitution in $\l$-calculus.
\end{proof}

\begin{theorem}
If $\Deri \Gamma M A$ then $M\in\SN{}$.
\end{theorem}
\begin{proof}
By Lemma~\ref{lem:typpreserved} and the strong normalisation of the
simply-typed $\l$-calculus, $M\in\bounded$ so $M\in\SN{}$ by
Corollary~\ref{cor:yahoo}.
\end{proof}

==> LexAdjournment.tex <==
\begin{definition}[Lexicographic reduction]
Let $\mathcal A_1,\ldots,\mathcal A_n$ be sets, \linebreak respectively equipped with the
reduction relations $\rightarrow_{\mathcal
A_1},\ldots,\rightarrow_{\mathcal A_n}$.

For $1\leq i\leq n$, let $\rightarrow_i$ be the reduction relation on
$\mathcal A_1\times\cdots\times\mathcal A_n$ defined as follows:
$$(M_1,\ldots,M_n)\rightarrow_i(N_1,\ldots,N_n)$$ if
$M_i\rightarrow_{\mathcal A_i}N_i$ and for all $1\leq j<i$, $M_j=N_j$ and
for all $i<j\leq n$, $N_j\in\SN{\rightarrow_{\mathcal A_j}}$.
We define the \emph{lexicographic reduction} 
$$\rightarrow_{\lex}
=\bigcup_{1\leq i\leq n}\rightarrow_i
$$
We sometimes write $\gllex[\rightarrow]$ for
${\glex[\rightarrow]}^+$, \ie the transitive closure of
$\glex[\rightarrow]$.
\end{definition}


\begin{corollary}[Lexicographic termination 1]\label{cor:lexic}$ $\\
$$\SN{\rightarrow_{A_1}}\times\cdots\times\SN{\rightarrow_{A_n}}\subseteq\SN{\rightarrow_{\lex}}$$
In particular, if $\rightarrow_{\mathcal
A_i}$ is terminating on $\mathcal A_i$  for all $1\leq i\leq n$, then $\rightarrow_{\textsf
{lex}}$ is terminating on
$\mathcal A_1\times\cdots\times\mathcal A_n$.
\end{corollary}

\begin{corollary}[Lexicographic termination 2]\label{cor:lexico}
Let $\mathcal A$ be a set equipped with a reduction relation
$\rightarrow$.

For each natural number $n$, let $\rightarrow_{\lex n}$ be the
lexicographic reduction on $\mathcal A^n$.

Consider the reduction relation $\rightarrow_{\lex}=\bigcup_n
\rightarrow_{\lex n}$ on the disjoint union $\bigcup_n \mathcal A^n$.

$$\bigcup_n (\SN{\rightarrow})^n\subseteq \SN{\rightarrow_\lex}$$
\end{corollary}

\begin{corollary}[Lexicographic simulation
  technique]\label{Cor:Simulation}
Let $\rightarrow_{\mathcal A}$
and $\rightarrow'_{\mathcal A}$ be two reduction relations on
$\mathcal A$, and $\rightarrow_{\mathcal B}$ be a reduction
relation on $\mathcal B$. Suppose
\begin{itemize}
\item
$\rightarrow'_{\mathcal A}$ is strongly simulated by
$\rightarrow_{\mathcal B}$ through $\mathcal R$
\item
$\rightarrow_{\mathcal A}$ is weakly simulated by
$\rightarrow_{\mathcal B}$ through $\mathcal R$
\item
$\SN{\rightarrow_{\mathcal A}}=\mathcal A$
\end{itemize}
Then $\mathcal R^{-1}(\SN{\rightarrow_{\mathcal
B}})\subseteq\SN{\rightarrow_{\mathcal
A}\cup\rightarrow'_{\mathcal A}}$.
\end{corollary}

\subsection{Adjournment in the framework of~\cite{LengrandPhD}}

\begin{definition}
Let $\rightarrow_1$ and $\rightarrow_2$ be two reduction relations on
$\mathcal A$.\\
The relation $\rightarrow_1$ can be \emph{adjourned with respect to}
$\rightarrow_2$ if\\ whenever $M\rightarrow_1 N \rightarrow_2 P$ there
exists $Q$ such that $M\rightarrow_2 Q (\rightarrow_1\cup\rightarrow_2)^* P$.
\end{definition}

\begin{theorem}
Let $\rightarrow_1$ and $\rightarrow_2$ be two reduction relations on
$\mathcal A$.\\ If $\rightarrow_1$ is terminating and can be adjourned
with respect to $\rightarrow_2$ then
$\SN{\rightarrow_2}\subseteq\SN{\rightarrow_1\cup\rightarrow_2}$.
\end{theorem}
\begin{proof}
First, we prove that $\rightarrow_2$ is strongly simulated by itself through
$({}_1\!\!\leftarrow\cup\ {}_2\!\!\leftarrow)^*$.

This means that, for all $k$, if
$M(\rightarrow_1\cup\rightarrow_2)^k N \rightarrow_2 P$ there
exists $Q$ such that $M\rightarrow_2 Q
(\rightarrow_1\cup\rightarrow_2)^* P$.  This is obtained by induction
on $k$:
\begin{itemize}
\item
If $k=0$, then take $Q=P$.
\item  Suppose the property is true for
some $k$, and suppose $M(\rightarrow_1\cup\rightarrow_2) N'
(\rightarrow_1\cup\rightarrow_2)^k N\rightarrow_2 P$.
\begin{itemize}
\item If $M\rightarrow_2 N' (\rightarrow_1\cup\rightarrow_2)^k
N\rightarrow_2 P$, then take $Q=N'$.
\item  If $M\rightarrow_1 N'
(\rightarrow_1\cup\rightarrow_2)^k N\rightarrow_2 P$, then use the
induction hypothesis on $N',N,P$ to get a $Q'$ such that
$M\rightarrow_1 N' \rightarrow_2 Q'(\rightarrow_1\cup\rightarrow_2)^*
P$. The adjournment hypothesis then gives $Q$ such that
$M\rightarrow_2 Q (\rightarrow_1\cup\rightarrow_2)^*
Q'(\rightarrow_1\cup\rightarrow_2)^k P$.
\end{itemize}
\end{itemize}
Second, $\rightarrow_1$ is weakly simulated by
$\rightarrow_2$ through $({}_1\!\!\leftarrow\cup\
{}_2\!\!\leftarrow)^*$: this just means that if
$M(\rightarrow_1\cup\rightarrow_2)^* N \rightarrow_1 P$ there exists
$Q$ such that $M\rightarrow^*_2 Q (\rightarrow_1\cup\rightarrow_2)^*
P$ (obtained by taking $Q=M$).

It then suffices to apply Corollary 26 of~\cite{LengrandPhD} (Corollary~\ref{Cor:Simulation}) to get that 
$(\rightarrow_1\cup\rightarrow_2)^*(\SN{\rightarrow_2})\subseteq\SN{\rightarrow_1\cup\rightarrow_2}$.
In particular, $\SN{\rightarrow_2}\subseteq\SN{\rightarrow_1\cup\rightarrow_2}$.
\end{proof}

